Structural Extensions of Basis Pursuit: Guarantees on Adversarial Robustness

While deep neural networks are sensitive to adversarial noise, sparse coding using the Basis Pursuit (BP) method is robust against such attacks, including its multi-layer extensions. We prove that the stability theorem of BP holds upon the following generalizations: (i) the regularization procedure can be separated into disjoint groups with different weights, (ii) neurons or full layers may form groups, and (iii) the regularizer takes various generalized forms of the $\ell_1$ norm. This result provides the proof for the architectural generalizations of Cazenavette et al. (2021), including (iv) an approximation of the complete architecture as a shallow sparse coding network. Due to this approximation, we settled to experimenting with shallow networks and studied their robustness against the Iterative Fast Gradient Sign Method on a synthetic dataset and MNIST. We introduce classification based on the $\ell_2$ norms of the groups and show numerically that it can be accurate and offers considerable speedups. In this family, linear transformer shows the best performance. Based on the theoretical results and the numerical simulations, we highlight numerical matters that may improve performance further.

==> bib_bib <==
@article{goodfellow2014explaining,
  title={Explaining and harnessing adversarial examples},
  author={Goodfellow, Ian J and Shlens, Jonathon and Szegedy, Christian},
  journal={arXiv preprint arXiv:1412.6572},
  year={2014}
}

@inproceedings{megyeri2021robust,
  title={Robust Classification Combined with Robust out-of-Distribution Detection: An Empirical Analysis},
  author={Megyeri, Istv{\'a}n and Heged{\"u}s, Istv{\'a}n and Jelasity, M{\'a}rk},
  booktitle={2021 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2021},
  organization={IEEE}
}

@article{kurakin2016adversarial,
  title={Adversarial Examples in the Physical World},
  author={Kurakin, Alexey and Goodfellow, Ian J and Bengio, Samy},
  journal={arXiv preprint arXiv:1607.02533},
  year={2016}
}

@inproceedings{katharopoulos2020transformers,
  title={Transformers are rnns: Fast autoregressive transformers with linear attention},
  author={Katharopoulos, Angelos and Vyas, Apoorv and Pappas, Nikolaos and Fleuret, Fran{\c{c}}ois},
  booktitle={International Conference on Machine Learning},
  pages={5156--5165},
  year={2020},
  organization={PMLR}
}

@inproceedings{arora2015simple,
  title={Simple, efficient, and neural algorithms for sparse coding},
  author={Arora, Sanjeev and Ge, Rong and Ma, Tengyu and Moitra, Ankur},
  booktitle={Conference on Learning Theory},
  pages={113--149},
  year={2015},
  organization={PMLR}
}

@inproceedings{naseer2020self,
  title={A self-supervised approach for adversarial robustness},
  author={Naseer, Muzammal and Khan, Salman and Hayat, Munawar and Khan, Fahad Shahbaz and Porikli, Fatih},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={262--271},
  year={2020}
}

@article{akhtar2021advances,
  title={Advances in adversarial attacks and defenses in computer vision: A survey},
  author={Akhtar, Naveed and Mian, Ajmal and Kardan, Navid and Shah, Mubarak},
  journal={IEEE Access},
  volume={9},
  pages={155161--155196},
  year={2021},
  publisher={IEEE}
}

@inproceedings{sulam2020adversarial,
 author = {Sulam, Jeremias and Muthukumar, Ramchandran and Arora, Raman},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M. F. Balcan and H. Lin},
 pages = {2110--2121},
 publisher = {Curran Associates, Inc.},
 title = {Adversarial Robustness of Supervised Sparse Coding},
 url = {https://proceedings.neurips.cc/paper/2020/file/170f6aa36530c364b77ddf83a84e7351-Paper.pdf},
 volume = {33},
 year = {2020}
}


@inproceedings{murdock2020dataless,
  title={Dataless model selection with the deep frame potential},
  author={Murdock, Calvin and Lucey, Simon},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11257--11265},
  year={2020}
}


@misc{AppA,
  title={Supplementary},
  author={Anonymous},
}

@article{murdock2021reframing,
  title={Reframing Neural Networks: Deep Structure in Overcomplete Representations},
  author={Murdock, Calvin and Lucey, Simon},
  journal={arXiv preprint arXiv:2103.05804},
  year={2021}
}

@article{liu2016delving,
  title={Delving into transferable adversarial examples and black-box attacks},
  author={Liu, Yanpei and Chen, Xinyun and Liu, Chang and Song, Dawn},
  journal={arXiv preprint arXiv:1611.02770},
  year={2016}
}

@inproceedings{cazenavette2020architectural,
  title={Architectural adversarial robustness: The case for deep pursuit},
  author={Cazenavette, George and Murdock, Calvin and Lucey, Simon},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7150--7158},
  year={2021}
}

@article{romano2020adversarial,
  title={Adversarial noise attacks of deep learning architectures: Stability analysis via sparse-modeled signals},
  author={Romano, Yaniv and Aberdam, Aviad and Sulam, Jeremias and Elad, Michael},
  journal={Journal of Mathematical Imaging and Vision},
  volume={62},
  number={3},
  pages={313--327},
  year={2020},
  publisher={Springer}
}

@inproceedings{szeghy2021adversarial,
  title={Adversarial Perturbation Stability of the Layered Group Basis Pursuit},
  author={Szeghy, D{\'a}vid and Milacski, Zolt{\'a}n A and F{\'o}thi, \'Aron and L{\H o}rincz, Andr{\'a}s},
  booktitle={Conference on Mathematics of Machine Learning, Max-Planck Institute für Mathematik},
  year = {2021},
}

@article{lorincz2016columnar,
  title={Columnar Machine: \mbox{F}ast estimation of structured sparse codes},
  author={L{\H{o}}rincz, Andr{\'a}s and Milacski, Zolt\'an A and Pint\'er, Bal\'azs and Ver{\H{o}}, Anita L},
  journal={Biologically Inspired Cognitive Architectures},
  volume={15},
  pages={19--33},
  year={2016},
  publisher={Elsevier}
}

@article{dhillon2008constructing,
  title={Constructing {P}ackings in {G}rassmannian {M}anifolds via {A}lternating {P}rojection},
  author={Dhillon, Inderjit S and Heath, Jr RW and Strohmer, Thomas and Tropp, Joel A},
  journal={Experimental Mathematics},
  volume={17},
  number={1},
  pages={9--35},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{fuchs2004sparse,
  title={On {S}parse {R}epresentations in {A}rbitrary {R}edundant {B}ases},
  author={Fuchs, J-J},
  journal={IEEE Trans. Inf. Theory},
  volume={50},
  number={6},
  pages={1341--1344},
  year={2004},
  publisher={IEEE}
}

@article{salehi2021unified,
  title={A Unified Survey on Anomaly, Novelty, Open-Set, and Out-of-Distribution Detection: Solutions and Future Challenges},
  author={Salehi, Mohammadreza and Mirzaei, Hossein and Hendrycks, Dan and Li, Yixuan and Rohban, Mohammad Hossein and Sabokrou, Mohammad},
  journal={arXiv preprint arXiv:2110.14051},
  year={2021}
}

@article{papyan2017working,
  title={{W}orking {L}ocally {T}hinking {G}lobally: {T}heoretical {G}uarantees for {C}onvolutional {S}parse {C}oding},
  author={Papyan, Vardan and Sulam, Jeremias and Elad, Michael},
  journal={IEEE Trans. Signal Process.},
  volume={65},
  number={21},
  pages={5687--5701},
  year={2017},
  publisher={IEEE}
}

@article{papyan2016working,
  title={Working {L}ocally {T}hinking {G}lobally-{P}art {II}: {S}tability and {A}lgorithms for {C}onvolutional {S}parse {C}oding},
  author={Papyan, Vardan and Sulam, Jeremias and Elad, Michael},
  journal={arXiv preprint arXiv:1607.02009},
  year={2016}
}

@article{papyan2017convolutional,
  title={{C}onvolutional {N}eural {N}etworks {A}nalyzed via {C}onvolutional {S}parse {C}oding},
  author={Papyan, Vardan and Romano, Yaniv and Elad, Michael},
  journal={J. Mach. Learn. Res.},
  volume={18},
  number={1},
  pages={2887--2938},
  year={2017},
  publisher={JMLR.org}
}

@article{tropp2006just,
  title={{J}ust {R}elax: {C}onvex {P}rogramming {M}ethods for {I}dentifying {S}parse {S}ignals in {N}oise},
  author={Tropp, Joel A},
  journal={IEEE Trans. Inf. Theory},
  volume={52},
  number={3},
  pages={1030--1051},
  year={2006},
  publisher={IEEE}
}


@inproceedings{gregor2010learning,
  title={Learning fast approximations of sparse coding},
  author={Gregor, Karol and LeCun, Yann},
  booktitle={Proceedings of the 27th international conference on international conference on machine learning},
  pages={399--406},
  year={2010}
}


@article{lecun2015deep,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={Nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{krizhevsky2012imagenet,
  title={Image{N}et {C}lassification with {D}eep {C}onvolutional {N}eural {N}etworks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Adv. NeurIPS},
  volume={25},
  pages={1097--1105},
  year={2012}
}

@article{ren2015faster,
  title={Faster {R-CNN}: {T}owards {R}eal-{T}ime {O}bject {D}etection with {R}egion {P}roposal {N}etworks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={arXiv:1506.01497},
  year={2015}
}

@inproceedings{he2017mask,
  title={Mask {R-CNN}},
  author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proc. IEEE ICCV},
  pages={2961--2969},
  year={2017}
}

@article{szegedy2013intriguing,
  title={Intriguing properties of neural networks},
  author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
  journal={arXiv:1312.6199},
  year={2013}
}

@article{athalye2018robustness,
  title={On the {R}obustness of the {CVPR} 2018 {W}hite-{B}ox {A}dversarial {E}xample {D}efenses},
  author={Athalye, Anish and Carlini, Nicholas},
  journal={arXiv:1804.03286},
  year={2018}
}

@book{elad2010sparse,
  title={Sparse \& {R}edundant {R}epresentations and {T}heir {A}pplications in {S}ignal and {I}mage {P}rocessing},
  author={Elad, Michael},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{donoho2003optimally,
  title={Optimally sparse representation in general (nonorthogonal) dictionaries via $\ell_1$ minimization},
  author={Donoho, David L and Elad, Michael},
  journal={Proc. Natl. Acad. Sci.},
  volume={100},
  number={5},
  pages={2197--2202},
  year={2003},
  publisher={National Acad. Sciences}
}

@article{chen2001atomic,
  title={Atomic {D}ecomposition by {B}asis {P}ursuit},
  author={Chen, Scott Shaobing and Donoho, David L and Saunders, Michael A},
  journal={SIAM Review},
  volume={43},
  number={1},
  pages={129--159},
  year={2001},
  publisher={SIAM}
}

@article{tibshirani1996regression,
  title={Regression {S}hrinkage and {S}election via the {LASSO}},
  author={Tibshirani, Robert},
  journal={J. R. Stat. Soc. Series B (Methodol.)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={Wiley Online Library}
}

@article{yuan2006model,
  title={Model {S}election and {E}stimation in {R}egression with {G}rouped {V}ariables},
  author={Yuan, Ming and Lin, Yi},
  journal={J. R. Stat. Soc. Series B (Methodol.)},
  volume={68},
  number={1},
  pages={49--67},
  year={2006},
  publisher={Wiley Online Library}
}

@article{bach2011optimization,
  title={Optimization with {S}parsity-{I}nducing {P}enalties},
  author={Bach, Francis and Jenatton, Rodolphe and Mairal, Julien and Obozinski, Guillaume},
  journal={arXiv:1108.0775},
  year={2011}
}

@inproceedings{he2016deep,
  title={Deep {R}esidual {L}earning for {I}mage {R}ecognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proc. IEEE CVPR},
  pages={770--778},
  year={2016}
}

@article{paszke2019pytorch,
  title={Py{T}orch: {A}n {I}mperative {S}tyle, {H}igh-{P}erformance {D}eep {L}earning {L}ibrary},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={arXiv:1912.01703},
  year={2019}
}

@article{bottou2018optimization,
  title={Optimization {M}ethods for {L}arge-{S}cale {M}achine {L}earning},
  author={Bottou, L{\'e}on and Curtis, Frank E and Nocedal, Jorge},
  journal={Siam Review},
  volume={60},
  number={2},
  pages={223--311},
  year={2018},
  publisher={SIAM}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book{ abelson-et-al:scheme,
  author = "Harold Abelson and Gerald~Jay Sussman and Julie Sussman",
  title = "Structure and Interpretation of Computer Programs",
  publisher = "MIT Press",
  address = "Cambridge, Massachusetts",
  year = "1985"
}

@inproceedings{ bgf:Lixto,
  author = "Robert Baumgartner and Georg Gottlob and Sergio Flesca",
  title = "Visual Information Extraction with {Lixto}",
  booktitle = "Proceedings of the 27th International Conference on Very Large Databases",
  pages = "119--128",
  publisher = "Morgan Kaufmann",
  address = "Rome, Italy",
  month = "September",
  year = "2001"
}

@article{ gottlob:nonmon,
  author = "Georg Gottlob",
  title = "Complexity results for nonmonotonic logics",
  journal = "Journal of Logic and Computation",
  volume = "2",
  number = "3",
  pages = "397--425",
  month = "June",
  year = "1992"
}

@article{ gls:hypertrees,
  author = "Georg Gottlob and Nicola Leone and Francesco Scarcello",
  title = "Hypertree Decompositions and Tractable Queries",
  journal = "Journal of Computer and System Sciences",
  volume = "64",
  number = "3",
  pages = "579--627",
  month = "May",
  year = "2002"
}

@article{ levesque:functional-foundations,
  author = "Hector~J. Levesque",
  title = "Foundations of a functional approach to knowledge representation",
  journal = "Artificial Intelligence",
  volume = "23",
  number = "2",
  pages = "155--212",
  month = "July",
  year = "1984"
}

@inproceedings{ levesque:belief,
  author = "Hector~J. Levesque",
  title = "A logic of implicit and explicit belief",
  booktitle = "Proceedings of the Fourth National Conference on Artificial Intelligence",
  publisher = "American Association for Artificial Intelligence",
  pages = "198--202",
  address = "Austin, Texas",
  month = "August",
  year = "1984"
}

@article{ nebel:jair-2000,
  author = "Bernhard Nebel",
  title = "On the compilability and expressive power of propositional planning formalisms",
  journal = "Journal of Artificial Intelligence Research",
  volume = "12",
  pages = "271--315",
  year = "2000"
}

 @misc{proceedings,
  author = {{IJCAI Proceedings}},
  title = {{IJCAI} Camera Ready Submission},
  howpublished = {\url{https://proceedings.ijcai.org/info}},
}

